A Complete framework for ambush avoidance in realistic environments

Operating vehicles in adversarial environments between a recurring origin-destination pair requires new planning techniques. A two players zero-sum game is introduced. The goal of the first player is to minimize the expected casualties undergone by a convoy. The goal of the second player is to maximize this damage. The outcome of the game is obtained via a linear program that solves the corresponding minmax optimization problem over this outcome. Different environment models are defined in order to compute routing strategies over unstructured environments. To compare these methods for increasingly accurate representations of the environment, a grid-based model is chosen to represent the environment and the existence of a sufficient network size is highlighted. A global framework for the generation of realistic routing strategies between any two points is described. This framework requires a good assessment of the potential casualties at any location, therefore the most important parameters are identified. Finally the framework is tested on real world environments.

==> sec_annexe.tex <==
\nblue{add A and Dk matrices relative to Figure \ref{fig:simple_ex} for better understanding}

\begin{figure*}
\setcounter{MaxMatrixCols}{20}
%\color{lightgray}
\begin{equation}
A = \begin{bmatrix}
	-1&-1&-1& 0& 0& 0& 0& 0& 0& 0& 0& 0& 0\\
     1& 0& 0&-1&-1& 0& 0& 0& 0& 0& 0& 0& 0\\
     0& 0& 0& 1& 0&-1& 1& 0& 0& 0& 0& 0& 0\\
     0& 1& 0& 0& 0& 0&-1&-1&-1& 0& 0& 0& 0\\
     0& 0& 0& 0& 1& 0& 0& 1& 0&-1& 1& 0& 0\\
     0& 0& 1& 0& 0& 0& 0& 0& 0& 0&-1&-1& 0\\
     0& 0& 0& 0& 0& 0& 0& 0& 1& 0& 0& 1&-1\\
     0& 0& 0& 0& 0& 1& 0& 0& 0& 1& 0& 0& 1\\
\end{bmatrix}\quad
b = \begin{bmatrix}
    -1\\
     0\\
     0\\
     0\\
     0\\
     0\\
     0\\
     1
\end{bmatrix}
\label{eq:Ab_ex}
\end{equation}

\begin{equation}
D_k = \begin{bmatrix}
	 0&0&0&0&0&0&0&0&0&0&0&0&0\\
	 1&0&0&0&0&0&0&0&0&0&0&0&0\\
     0&0&0&1&0&0&1&0&0&0&0&0&0\\
     0&1&0&0&0&0&0&0&0&0&0&0&0\\
     0&0&0&0&1&0&0&1&0&0&1&0&0\\
     0&0&1&0&0&0&0&0&0&0&0&0&0\\
     0&0&0&0&0&0&0&0&1&0&0&1&0\\
     0&0&0&0&0&0&0&0&0&0&0&0&0
\end{bmatrix}
\label{eq:dk_ex}
\end{equation}
%\color{black}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Glossary}

\begin{itemize}
\item scenario: environnement + mission + carte de cout
\item method: pr construire le reseau
\item "risk": combien on perd
\item "entropy": $\sum \limits_{i,j | (i,j) \in \mathcal{E}} p_{ij}log(p_{ij})$
\item ???: ambush type method
\end{itemize}


==> sec_risk.tex <==
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	\subsection{Definition of risk}
%\nblue{see risk paper "On the quantitative definition of risk"}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\subsection{Risk factors}

\nblue{Environmental Risk (risk diagram)}

In order to extend the purely theoretical game theory problem and make it more realistic, interviews of former Army personnel were performed. The focus of these interviews was to identify the factors with the highest influence on risks that could be incorporated into the optimization problem formulation. \red{on a mis un accent tout particulier sur l'identification des facteurs de risques a prendre en compte}.

 \aude{ecoute les fichiers audio dans Notes/Justin... pr mieux comprendre (en vitesse 1.5x)}

The relevant information can be categorized into three different areas. First, the information related to the environment, whether described by topological or geospatial data is decisive. Second, the strategical information \aude{explain?} needs to be taken into account. Third, the human factors matter for... \aude{details?}. 

It should be noted that these categories are correlated. For example, for a given type of vehicle, what is the strategic information, the maximum speed of this vehicle depends on the topology of the environment: a jeep might be faster than a human on a road but not inside a dense forest.
	
\nred{need new diagram for risk with 3 categories}

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=6in,height=4in]{risk_diagram.png}
\caption{Different factors to consider for risk computation at a given location.}
\label{fig:risk_diagram}
\end{center}
\end{figure}
	
\nblue{Wrap up: key factors. vision range + vision quality + maximum speed. How fast can I detect danger and how fast I can move react/move.}
\aude{key factors for what? each player? how can you incorporate these?}

In order to minimize the possible casualties, we need to predict the risk from far away and be able to escape fast. \aude{far away spatially or as early as possible? look-ahead time?}

\nblue{Conclusion: we have identified risk factors. ??? }


\nblue{"Risk map" depends on mission (strategical information)}
\aude{The structure of the risk map depends on the type of mission studied. It is part of the overall strategic information. The three main items ...}
\blue{ 
\begin{itemize}
\item scout: uniform (if we're seen, we loose)
\item transport: depends on environment
\item patrol: depends on environment but DIFFERENT from transport (there could be a positive outcome in being ambushed since we want to flush RED out)
\end{itemize}
}
